Derived Semidistributive Lattices

For L a finite lattice, let C(L) denote the set of pairs g = (g_0,g_1) such that g_0 is a lower cover of g_1 and order it as follows: g <= d iff g_0 <= d_0, g_1 <= d_1, but not g_1 <= d_0. Let C(L,g) denote the connected component of g in this poset. Our main result states that C(L,g) is a semidistributive lattice if L is semidistributive, and that C(L,g) is a bounded lattice if L is bounded. Let S_n be the permutohedron on n letters and T_n be the associahedron on n+1 letters. Explicit computations show that C(S_n,a) = S_{n-1} and C(T_n,a) = T_{n-1}, up to isomorphism, whenever a is an atom. These results are consequences of new characterizations of finite join semidistributive and finite lower bounded lattices: (i) a finite lattice is join semidistributive if and only if the projection sending g in C(L) to g_0 in L creates pullbacks, (ii) a finite join semidistributive lattice is lower bounded if and only if it has a strict facet labelling. Strict facet labellings, as defined here, are generalization of the tools used by Barbut et al. to prove that lattices of Coxeter groups are bounded.

==> macros.tex <==
\RequirePackage{ifthen}


%% Theorems
\newcommand{\eproofofclaimlabel}{\mbox{$\Box$\hspace{2mm}\emph{Claim}}}
\newcommand{\eproofofclaim}{%
  \mbox{\hspace{1mm}}~\hfill\eproofofclaimlabel\par\vskip6pt}

\newlength{\misslen}
\newlength{\misslend}
\newcommand{\miss}[1]{%
  % \ifthenelse{\equal{#1}{i}}{%
%     \text{{\it \^{i}}}
%   }{%
      \settowidth{\misslen}{\mbox{$k$}}
      \settowidth{\misslend}{\mbox{$#1$}}
      \ifthenelse{\lengthtest{\misslen<\misslend}}%
      {\widehat{#1}}%
      {\hat{#1}}%
      % }
}
\newcommand{\missi}{\text{{\it \^{i}}}}

\newcommand{\double}[1]{N^{#1}}

\newcommand{\enumref}[1]{\emph{(#1)}}

\newcommand{\pr}[1][0]{(\,\cdot \,)_{#1}}

%\newcommand{\Precubes}{p\mathcal{C}ubes}
\newcommand{\Perm}{\mathcal{P}erms}

%% Special Order
\newcommand{\spushdown}[2][0pt]{\pushdown[\!\raisebox{#1}{${}_{#2}$}]}

%% Text Logic
\newcommand{\tand}{\text{ and }}
\newcommand{\tif}{\text{ if }}
\newcommand{\tiff}{\text{ iff }}
\newcommand{\toth}{\text{otherwise}}
\newcommand{\timplies}{\text{ implies }}

%% Calligraphcs
\newcommand{\Am}{\sqrt{\!\!A}}
%\newcommand{\Am}{A^{\sqrt{\cdot}}}
\newcommand{\cAm}{{\cal A}}
\newcommand{\cBm}{{\cal B}}

\newcommand{\breath}{\vskip 6pt}

%% XY

\newgraphescape{c}[1]{%
  []*+{#1{}_{0}}="#1_{0}"
  -[u]*+{#1{}_{1}}="#1_{1}"
  |{}="#1_{m}"
  "#1_{0}"
}

\newgraphescape{d}[2]{%
  []!~:{@{.}}
  []*+{#2_{0}}="#2_{0}"-[u(1)l(#1)]*+{#2_{1}}="#2_{1}"|{}="#2_{m}"
  "#2_{0}"
}

\newgraphescape{e}[2]{%
  []!~:{@{.}}
  []("#1_{0}":"#2_{0}",
  "#1_{1}":"#2_{1}")
}

\newdir{++}{{}*!/3pt/\dir{+}{}*!/3pt/\dir{-}}

\newgraphescape{p}[3]{%
  !~:{@{.}}
  "#1_{0}":"#2_{0}"
  "#1_{1}":@{{ }{ }{ }}@/-1em/"#2_{1}"|{}="i"
  %
  "#1_{1}"-"i"*+{#3}:"#2_{1}"
  %
  %"#2_{1}":"#1_{0}"
  []!~:{@{ ->}}
}

\newgraphescape{u}[3]{%
  !~:{@{.}}
  "#1_{1}":"#2_{1}"
  "#2_{0}":@{{ }{ }{}}@/-0.1em/"#1_{0}"|{}="i"
  "#1_{0}":"i"*+{#3}-"#2_{0}"
}

\newgraphescape{f}[4]{%
  [](
  "#2":@{{.}{.}{.}}@/#4/"#3"|*+{#1}
  )
}

\newgraphescape{g}{%
  [](
  []*+{\scriptstyle{i}}="i0"
  ([d]="i1"[d]="i2"[d]*+{\scriptstyle{i}}="i3")
  [r]*+{\scriptstyle{i+1}}="j0"([d]="j1"[d]="j2"
  [d]*+{\scriptstyle{i+1}}="j3")
  [r]="k0"([d]="k1"[d]="k2"[d]*+{\scriptstyle{i+2}}="k3")
  )
  "i1":@{.}"k1"
  "i2":@{.}"k2"
}

\newgraphescape{h}{%
  [](
  []*+{\scriptstyle{i}}="i0"([d]="i1"[d]*+{\scriptstyle{i}}="i2")
    [r]*+{\scriptstyle{i+1}}="j0"([d]="j1"[d]*+{\scriptstyle{i+1}}="j2")
    [r]="k0"([d]="k1"[d]*+{\scriptstyle{i+2}}="k2")
  )
  "i1":@{.}"k1"
}

\newgraphescape{G}{%
  [](
  []*+{\scriptstyle{i-1}}="i0"
  ([d]="i1"[d]="i2"[d]*+{\scriptstyle{i-1}}="i3")
  [r]*+{\scriptstyle{i}}="j0"([d]="j1"[d]="j2"
  [d]*+{\scriptstyle{i}}="j3")
  [r]="k0"([d]="k1"[d]="k2"[d]*+{\scriptstyle{i+1}}="k3")
  )
  "i1":@{.}"k1"
  "i2":@{.}"k2"
}

\newgraphescape{H}{%
  [](
  []*+{\scriptstyle{i-1}}="i0"([d]="i1"[d]*+{\scriptstyle{i-1}}="i2")
    [r]*+{\scriptstyle{i}}="j0"([d]="j1"[d]*+{\scriptstyle{i}}="j2")
    [r]="k0"([d]="k1"[d]*+{\scriptstyle{i+1}}="k2")
  )
  "i1":@{.}"k1"
}

\newgraphescape{k}{
  [d(0.5)]*+{}*\cir{}
}

\newgraphescape{t}[2]{%
  []="SE#1"(
  -[u(#2)]="NO#1"
  -[r(#2)]="NE#1",
  "SE#1"-"NE#1"
  )
  "SE#1"[d(0.3)]*[r]+{#1}
}

\newcommand{\mydiagram}[2][6em]{
  \mbox{$\begin{array}{@{\hspace{0mm}}c@{\hspace{0mm}}}
      \xy\xygraph{!{<#1,0cm>:<0cm,#1>::}#2}\endxy
    \end{array}$}
  }





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "0"
%%% End: 

